MPC without Terminal Ingredients Tailored to the SEIR Compartmental Epidemic Model

We consider the SEIR compartmental epidemic model subject to state and input constraints (a cap on the proportion of infectious individuals and limits on the allowed social distancing and quarantining measures, respectively). We present a tailored model predictive control (MPC) scheme without terminal conditions. We rigorously show recursive feasibility and asymptotic convergence of the MPC closed loop to the continuum of disease-free equilibrium points for suitably designed quadratic running cost and a sufficiently long prediction horizon (forecast window). Moreover, we establish the viability kernel (a.k.a. the admissible set) as a domain of attraction of the continuum of equilibria.

==> tex/cost_controllability.tex <==
\section{MPC without Terminal Cost or Target}
Consider the finite-horizon optimal control problem:
\[
\OCPT : \quad \inf_{u \in \U_T(x_0)} J_T(x_0,u),
\]
with cost functional,
\[
	J_T(x_0,u) := \int_0^T \ell(x(s;x_0,u),u(s))\,\dee s,
\]
and stage costs $\ell : \mathbb{R}^n \times \mathbb{R}^m \to \mathbb{R}$, 
\begin{equation}
	\ell(x,u) := E^2 + I^2 + (\beta - \beta_{\nom})^2 + (\gamma - \gamma_{\nom})^2. \label{quadratic_ell}
\end{equation}
The set $\U_T(x_0)$ denotes all control functions $u \in \U$ for which $x(t;x_0,u)\in G_{\Pi}$ for all $t \in [0,T]$. 
Note that in contrast to~\cite{SaueEste22} there are no terminal costs or constraints. 
The value function is given by:
\[
	V_T(x_0):= \inf_{u\in\U_T(x_0)} J_T(x_0,u).
\]
We define the set 
\[
	\A^{\prime}_{\nom} := \A \setminus\mathcal{N}(\mathcal{E}^{\prime}_{\nom},\epsilon).
\]
\begin{remark}\label{rem:continuum_of_equilibria}
	In contrast to classical MPC, where the aim is to drive the system to a particular controlled equilibrium~$\bar x$, see e.g.~\cite{esterhuizen2020recursive}, our goal is to reach any point within the continuum $\mathcal{E}_\mathrm{nom}$. % 
\end{remark}
\begin{lemma}
	$V_{\infty}(x_0)<\infty$ for all $x_0\in\A^{\prime}$.
\end{lemma}
\begin{proof}
	See proof of Lemma 4 from ECC paper, but I think this needs to be improved.
\end{proof}



Let's show that MPC without stabilising ingredients ``works'' from any initial condition in $\A^{\prime}$ with a sufficiently long finite prediction horizon $T>0$. To this end we will use the following two boxes:
\[
	\XM := \{(S,E,I):S \leq \frac{\gamma_{\nom}}{\beta_{\nom}}, E\leq \frac{\gamma_{\nom}I_{\max}}{\eta}, I\leq I_{\max}\},
\]
\[
	\XA := \{(S,E,I):S \leq \frac{\gamma_{\max}}{\beta_{\min}}, E\leq \frac{\gamma_{\max}I_{\max}}{\eta}, I\leq I_{\max}\}.
\]
\begin{lemma}
	\begin{itemize}
		\item $\XM\subseteq\M$ and for any $x_0\in\XM$, with $u(t)\equiv u_{\nom}:=(\beta_{\nom},\gamma_{\nom})^\top$, $\XM$ is invariant, and $E$ and $I$ {\color{blue}decay exponentially}.
		\item $\XA\subseteq\A$ and for any $x_0\in\XA$, with $u(t)\equiv \hat{u}:=(\beta_{\min},\gamma_{\max})^\top$, $\XA$ is invariant, and $E$ and $I$ {\color{blue}decay exponentially}. 
	\end{itemize}
\end{lemma}
\begin{proof}
	Focusing on $\XM$, let $g_1(x) := S - \frac{\gamma_{\nom}}{\beta_{\nom}}$, $g_2(x) := E - \frac{\gamma_{\nom}I_{\max}}{\eta}$ and $g_3(x) := I - I_{\max}$. Let $\mathbb{I}(x)\subseteq\{1,2,3\}$ denote the indices of active constraints at the state $x$. Now consider the Lie derivative at any $x_0\in\partial \XM$. We see that, for $x\in\partial\XM$ and $S = \frac{\gamma_{\nom}}{\beta_{\nom}}$,
	\begin{align*}
		L_f g_1(x,u_{\nom}) = -\beta_{\nom}\frac{\gamma_{\nom}}{\beta_{\nom}}I < 0.
	\end{align*}
	For $x\in\partial\XM$ and $E = \frac{\gamma_{\nom}I_{\max}}{\eta}$,
	\begin{align*}
		L_f g_2(x,u_{\nom}) = \beta_{\nom}SI -\eta E = \beta_{\nom}SI -\eta \frac{\gamma_{\nom}I_{\max}}{\eta} = \beta_{\nom}SI - \gamma_{\nom}I_{\max}\leq \gamma_{\nom}(I - I_{\max})\leq 0.
	\end{align*}
	For $x\in\partial\XM$ and $I = I_{\max}$,
	\begin{align*}
		L_f g_3(x,u_{\nom}) = \eta E - \gamma_{\nom} I_{\max} = \gamma_{\nom}I_{\max} - \gamma_{\nom} I_{\max} \leq 0.
	\end{align*}
	Therefore, for any $x\in\partial\XM$, with $u(t)\equiv u_{\nom}$,
	\begin{align*}
		\max_{i\in\mathbb{I}(x)}L_f g_i(x,u_{\nom}) \leq 0,
	\end{align*}
	and so $\XM$ is invariant under $u(t)\equiv u_{\nom}$. The proof that $E$ and $I$ {\color{blue}decay exponentially} was shown in Lemma 2 of ECC paper. The invariance of $\XA$ under $\hat{u}$, and exponential decay of $E$ and $I$ follow the same lines of reasoning.
\end{proof}

We now verify the three assumptions from the appendix. Assumption (A1) holds because the running cost is quadratic. %
However, as mentioned in Remark~\ref{rem:continuum_of_equilibria}, we need to adjust the definition to cope with the continuum of possible desired equilibria: 
\begin{align}
	\underline{\eta} \left( \left\| \begin{pmatrix} x_2 \\ x_3 \end{pmatrix} \right\|_2 \right) \; \leq \; \ell^\star(x) \; \leq \; \bar{\eta} \left( \left\| \begin{pmatrix} x_2 \\ x_3 \end{pmatrix} \right\|_2 \right) \quad \forall \, x \in X \notag 
\end{align}

Let's investigate (A2) (``cost controllability''). We show that cost controllability holds on the following $\epsilon$-neighbourhood of $\mathcal{E}_{\nom}$:
\[
	\mathcal{N}(\mathcal{E}_{\nom},\epsilon) := \{(S,E,I)^\top\in G_{\Pi} : S \leq \frac{\gamma_{\nom}}{\beta_{\nom}}, \min\{E, I\} < \epsilon\},
\]
\begin{proposition}
	There exists a $\rho<\infty$ such that $V_{\infty}(x_0)\leq \rho \ell^{\star}(x_0)$ for all $x_0\in\XM$.
\end{proposition}

\begin{proof}
	First, consider any $x_0\in\XM$, for which $S_0\leq\frac{\gamma_{\nom}}{\beta_{\nom}}$, with $u(t)\equiv u_{\nom}$. Then, because $S(t)$ is strictly decreasing w.r.t. time, $S(t) < \frac{\gamma_{\nom}}{\beta_{\nom}}$ for all $t> 0$ and $\dot{E}(t) + \dot{I}(t) = (\beta_{\nom}S(t) - \gamma_{\nom})I(t) < 0$ for all $t> 0$. Moreover, because $E(t) + I(t) \geq 0$ for all $t\geq 0$, $\frac{\dee}{\dee t}\left(E(t) + I(t)\right)^2 = 2\left(E(t) + I(t)\right)\left(\dot{E}(t) + \dot{I}(t)\right)< 0$ for all $t> 0$. 
	
	Therefore, noting that $0\leq E^2(t) + I^2(t) \leq (E(t) + I(t))^2\leq E(t) + I(t)\leq 1$ for all $t$, and $\lim_{t\rightarrow \infty} E(t) + I(t) = 0$, there exists a finite $t_1\geq 0$ such that $E^2(t_1) + I^2(t_1)\leq\left(E(t_1) + I(t_1)\right)^2 = \frac{1}{2}\left(E_0^2 + I_0^2\right)$, and there exists a finite $t_2\geq t_1$ such that $E^2(t_2) + I^2(t_2)\leq\left(E(t_2) + I(t_2)\right)^2 = \frac{1}{4}\left(E_0^2 + I_0^2\right)$, etc. (The dependence of the $t_i$'s on the initial condition $x_0$ are dropped to lighten the notation.)
	
	Recall that (from ECC paper), with $t_0 = 0$,
	\begin{align*}
		J_{\infty}(x_0,u_{\nom}) & = \int_0^{\infty} \left(E^2(s) + I^2(s) \right)\,\mathrm{d}s < \infty,\,\,x_0\in\XM.
	\end{align*}
	Moreover,
	\begin{align*}
	\sum_{n=1}^{\infty}\frac{1}{2^{n}}(t_n - t_{n-1})\left(E_0^2 + I_0^2\right) \leq &J_{\infty}(x_0,u_{\nom})\leq \sum_{n=1}^{\infty}\frac{1}{2^{n-1}}(t_n - t_{n-1})\left(E_0^2 + I_0^2\right).
	\end{align*}
	The series $\sum_{n=1}^{\infty}\frac{1}{2^{n-1}}(t_n - t_{n-1})$ converges, for if this were not true, the series $\sum_{n=1}^{\infty}\frac{1}{2^{n}}(t_n - t_{n-1})$ would diverge as well, which is impossible because $J_{\infty}(x_0,u_{\nom})<\infty$. {\WE (WE: Better argument?)} Therefore, for any $x_0\in\XM$ there exists a constant $\rho(x_0) := \lim_{k \to  \infty} \sum_{n=1}^{k} \frac{1}{2^{n-1}}(t_n - t_{n-1}) < \infty$. 
	Since the solution $x(t; x_0, u)$ at time $t \geq 0$ continuously depends on the initial value~$x_0$ for any $u \in \mathcal{U}$, see e.g.~\cite{XXX}, so does the time $t_k = t_k(x_0)$, $k \in \mathbb{N}$. %
	Therefore, $\rho$ is continuous. %
	Because $\XM$ is compact, %, there exists a $\bar \rho < \infty$, given by:
	\[
		\bar \rho := \max_{x_0 \in \XM} \rho(x_0) < \infty
	\]
	exists. %
	From Lemma~2, the set $\XM$ is invariant under $u(t) \equiv u_{\nom}$, meaning that $I(t) \leq I_{\max}$. Therefore,
	\[
		V_{\infty}(x_0)= \inf_{u\in\U_{\infty}(x_0)} J_{\infty}(x_0,u) \leq J_{\infty}(x_0,u_{\nom}) \leq \bar \rho \left( E_0^2 + I_0^2 \right) = \bar \rho \ell^{\star}(x_0), \quad \forall x_0 \in \XM.
	\]
\end{proof}
The following corollary then follows because $\mathcal{N}(\mathcal{E}_{\nom},\epsilon)\subseteq \XM$.
\begin{corollary}
	There exists a $\rho<\infty$ such that $V_{\infty}(x_0)\leq \rho \ell^{\star}(x_0)$ for all $x_0\in\mathcal{N}(\mathcal{E}_{\nom},\epsilon)$.
\end{corollary}

Now let's consider the points:
\[
	\hat{\mathcal{E}} :=\{(S,E,I): S < \frac{\gamma_{\max}}{\beta_{\min}}, E=I=0\}\subset\mathcal{E}.
\]
%\begin{proposition}
%	There exists a $\hat{\rho}<\infty$ such that $V_{\infty}(x_0)\leq \hat{\rho} \left(E_0^2 + I_0^2\right)$ for all $x_0\in\mathcal{N}(\hat{\mathcal{E}})\cap G_{\Pi}$. 
%	{\color{red}PS:\ This conjecture does not hold. %
\begin{remark}
	(A2) does not hold for equilibria $\bar x = (S, 0, 0)^\top$ with $S > \bar S$. % 
	Consider the equilibrium point $x^\star = (S^\star, 0, 0)^\top$ with $S^\star > \bar S := \gamma_\mathrm{nom} / \beta_\mathrm{nom}$ and $\varepsilon < S^\star - \bar S$. % 
	Then, for all $x_0 = (S_0, E_0, I_0) \in \mathcal{N}_\varepsilon(x^\star)$ with $\min \{E_0, I_0\} > 0$, the optimal value $V(x_0)$ is bounded away from~0 since $S_0 - \bar S$ many people have to get infected before we can drop the controls. %
	However, $\ell^\star(x_0)$ tends towards 0 for $E_0, I_0 \to 0$. 
\end{remark}
%	}
%\end{proposition}

%\begin{proof}
%	As in the proof of the previous Proposition, if $u(t)\equiv\hat{u}=(\gamma_{\max},\beta_{\min})^\top$, because $S_0<\frac{\gamma_{\max}}{\beta_{\min}}$ and $S(t)$ is strictly decreasing, $E(t) + I(t)$ and $\left(E(t) + I(t)\right)^2$ are strictly decreasing for $t\geq 0$. Moreover, $E^2(t) + I^2(t) \leq \left(E(t) + I(t)\right)^2\leq E(t) + I(t)\leq 1$, and $\lim_{t\rightarrow \infty} E(t) + I(t) = 0$. Thus, by the same arguments as before, there exists a constant $\rho<\infty$ such that
%	\[
%		\int_{0}^{\infty} E^2(s) + I^2(s)\,\dee s \leq \rho\ell^{\star}(x_0),\,\,\forall x_0\in\XA.
%	\]
%	Moreover, there exists a finite $\hat{t}\geq 0$, such that $E(\hat{t}) + I(\hat{t}) = \frac{\gamma_{\nom}I_{\max}}{\eta}>0$, thus $E(\hat{t}) \leq \frac{\gamma_{\nom}I_{\max}}{\eta}$ and $S(\hat{t}) \leq \frac{\gamma_{\nom}}{\beta_{\nom}}$ {\WE This is wrong.}. Also recall that, because $\XA$ is invariant under $u(t)\equiv \hat{u}$, $I(t)\leq I_{\max}$ for all $t\geq 0$. Thus, $x(\hat{t})\in\XM$. We can now define the control function: 
%	\[
%		\tilde{u}(t) = \hat{u},\,\,\mathrm{for}\,\,t\in[0,\hat{t}]
%	\]
%	\[
%		\tilde{u}(t) = u_{\nom},\,\,\mathrm{for}\,\,t\in[\hat{t},\infty).
%	\]
%	The resulting cost function, for any $x_0\in\XA$, is:
%	\begin{align*}
%		J_{\infty}(x_0,\tilde{u}) & = \int_0^{\infty} E^2(s) + I^2(s)\,\mathrm{d}s + \int_0^{\infty} (\beta(s) - \beta_{\nom})^2 + (\gamma(s) - \gamma_{\nom})^2\,\mathrm{d}s,\\
%		&\leq \rho\ell^{\star}(x_0) + \hat{\rho},
%	\end{align*}
%	where $\hat{\rho}:= \hat{t} \left[ (\beta_{\min} - \beta_{\nom})^2 + (\gamma_{\max} - \gamma_{\nom})^2 \right] = \int_0^{\hat{t}} (\beta_{\min} - \beta_{\nom})^2 + (\gamma_{\max} - \gamma_{\nom})^2\,\mathrm{d}s <\infty$. Now, define the new constant $\tilde{\rho}:= \frac{\hat{\rho}}{(E_0^2 + I_0^2)}$, for $x_0\in\XA\setminus \XM$. Note that $\tilde{\rho} < \infty$ because $E_0 > \frac{\gamma_{\nom}I_{\max}}{\eta}$. {\WE WE: no, rethink this... E0 can be small. The problem is that the left hand integral only involving the state is finite with $\tilde{u}$, but that the right hand one only involving the control blows up, which is fine. However, $u_{\nom}$ might actually work, in which case $V$ is not infinite.}
%	
%	Therefore, because the state constraint is satisfied for all $t$ under $\tilde{u}$,
%	\begin{align*}
%		V_{\infty}(x_0) & = \inf_{u\in\U_{\infty}(x_0)} J_{\infty}(x_0,u)\leq J_{\infty}(x_0,\tilde{u}) \leq \left(\rho + \tilde{\rho}\right)\ell^{\star}(x_0).
%	\end{align*}
%\end{proof}
%
%Now, we show that (A2) is violated for controlled equilibrium points satisfying $S_0 > \frac{\gamma_{\max}}{\beta_{\min}}$.
%
%\begin{proposition}
%	Consider a controlled equilibrium point $x_0\in\mathcal{E}\setminus \{(S,E,I): S \leq \frac{\gamma_{\max}}{\beta_{\min}}\}$. There exists a $\rho$ such that for every $\epsilon> 0$,
%	\[
%		V_{\infty}(x) > \rho \ell^{\star}(x),	
%	\]
%	for all $x\in\mathcal{N}(\hat{\mathcal{E}},\epsilon)\cap G_{\Pi}$.
%\end{proposition}
%
%\begin{proof}
%	{\WE WE: PROOF}
%\end{proof}

\begin{proposition}
	(A3) holds.
\end{proposition}
\begin{proof}
	Let $T > 0$ be given. % 
	Note that
	\begin{align}
		\dot E(t) \; & = \; \beta(t) S(t) I(t) - \eta E(t) \; \geq \; - \eta E(t) \notag \\
		\dot I(t) \; & = \; \eta E(t) - \gamma(t) I(t) \; \geq \; - \gamma_\mathrm{max} I(t) \notag 
	\end{align}
	and, thus, 
	\begin{align*}
		V_{\delta}(x_0) \; = \; \inf_u \int_0^{\delta} E^2(s) + I^2(s) \, \dee s \; & \geq \; \int_0^{\delta} e^{-2\eta t}E_0^2 + e^{-2 \gamma_\mathrm{max} t}I_0^2 \, \dee s \\
		& \geq \; \int_0^\delta \mathrm{e}^{-2 \eta \delta} E_0^2 + \mathrm{e}^{-2 \gamma_\mathrm{max} \delta} I_0^2 \, \dee s \\
		& \geq \; \int_0^\delta \mathrm{e}^{- 2 \delta \max \{ \eta, \gamma_\mathrm{max} \}} (E_0 + I_0^2) \, \dee s \\
		& \geq \; \mathrm{e}^{- 2 \delta \max \{ \eta, \gamma_\mathrm{max} \}} \delta \ell^\star(x_0) 
	\end{align*}	
	or, equivalently, 
	\begin{align}
		\bar C V_\delta(x_0) \; \geq \; \delta \ell^\star(x_0) \notag 
	\end{align}
	with $\bar C := \max_{\delta \in (0,T]} \mathrm{e}^{2 \delta \max \{ \eta, \gamma_\mathrm{max} \}} = \mathrm{e}^{ 2 T \max \{ \eta, \gamma_\mathrm{max} \}}$. %
\end{proof}

Thus, if $T>0$ is large enough, the state can be driven from any $x_0\in V_T^{-1}[0,C]$, $C>0$, to a controlled equilibrium on $\mathcal{E}$ for which $S_0 \leq \frac{\beta_{\nom}}{\gamma_{\nom}}$, via CT MPC without stabilising costs or constraints. The MPC closed-loop would be stable and the constraints would be satisfied for all time. (The state would be driven to an equilibrium point on $\mathcal{E}$, but this cannot be chosen beforehand.)

The MPC algorithm reads:
\begin{algorithm}[h]
	\caption{Continuous-time MPC}
	\noindent \textbf{Input}: time shift $\delta \in \mathbb{R}_{>0}$, $N \in \mathbb{N}$, initial state $x_0 \in \mathcal{A}^{\prime}$\\
	\textbf{Set}: prediction horizon $T \leftarrow N \delta$, $\hat{x} \leftarrow x_0$.
	\begin{enumerate}
		\item Find a minimizer $u^\star \in \arginf_{u \in \mathcal{U}_T(\hat{x})} J_T(\hat{x},u)$.
		\item Implement $u^\star(\cdot)$, for $t \in [0, \delta)$.
		\item Set $\hat{x}\leftarrow x(\delta;\hat{x},u^{\star})$ and go to step 1).
	\end{enumerate}
	\label{alg:mpc}
\end{algorithm}

\begin{proposition}
	There exists a finite $T> 0$ such that from any initial state $x_0\in\A^{\prime}$, $\OCPT$ is recursively feasible and the MPC closed loop is driven to an equilibrium point on $\mathcal{E}_{\nom}$.
	
	(In other words, with $T$ sufficiently large, $\A^{\prime}$ becomes the region of attraction of $\mathcal{E}_{\nom}$ under the MPC feedback.)
\end{proposition}
\begin{proof}
	We have verified that (A1) and (A3) hold. Moreover, (A2) (cost controllability) holds on $\mathcal{E}_{\nom}$. Thus, noting that $\A^{\prime}\subseteq V_T^{-1}[0,C]$ (recall from Lemma~1 that $V_{\infty}(x_0)$ is bounded on $\A^{\prime}$), the result follows from Theorem~1 of the appendix.
\end{proof}






==> tex/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
%\usepackage{amsthm}
\usepackage{color}
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{color}
\usepackage{braket} % allow for \Set{...}
\usepackage{algorithm}
\usepackage{cases}
\usepackage{array}



\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}
\newcommand{\red}{\color{red}}
\newcommand{\blk}{\color{black}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\boldv}{\mathbf{v}}
\newcommand{\bdot}{\textbf{.}}
\newcommand{\boldu}{\mathbf{u}}
\newcommand{\gnom}{\gamma_{\nom}}
\newcommand{\bnom}{\beta_{\nom}}
\newcommand{\sat}{\mathsf{sat}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\X}{\mathbb{X}}
\newcommand{\DAO}{[\partial \A]_{0}}
\newcommand{\DAM}{[\partial \A]_{-}}
\newcommand{\Int}{\mathsf{int}}
\newcommand{\ee}{\epsilon}
\newcommand{\dee}{\mathrm{d}}
\newcommand{\co}{\mathsf{co}}
\newcommand{\dist}{\mathsf{dist}}
\newcommand{\Cl}{\mathsf{cl}}
\newcommand{\nom}{\mathrm{nom}}
\newcommand{\OCPT}{\mathrm{OCP_T}}
\newcommand{\XM}{\mathbb{X}_{\mathcal{M}}}
\newcommand{\XA}{\mathbb{X}_{\mathcal{A}}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\WE}{\color{blue}}
\newcommand{\mbbR}{\mathbb{R}}
\newcommand{\argmin}{\mathrm{argmin}}
\newcommand{\term}{\mathrm{term}}
\newcommand{\fraku}{\mathfrak{u}}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
\newsiamthm{problemstatement}{Problem Statement}


% Sets running headers as well as PDF title and authors
\headers{MPC without Terminal Ingredients Tailored to SEIR Model}{W. Esterhuizen, P. Sauerteig, K. Worthmann, and S. Streif}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{MPC without Terminal Ingredients Tailored to the SEIR Compartmental Epidemic Model\thanks{Submitted to the editors DATE.
\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}

% Authors: full names plus addresses.
\author{Willem Esterhuizen\thanks{Imagination Corp., Chicago, IL 
  (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
\and Philipp Sauerteig\thanks{Department of Applied Mathematics, Fictional University, Boise, ID 
  (\email{ptfrank@fictional.edu}, \email{jesmith@fictional.edu}).}
\and Stefan Streif\thanks{Department of Applied Mathematics, Fictional University, Boise, ID 
	(\email{ptfrank@fictional.edu}, \email{jesmith@fictional.edu}).}
\and Karl Worthmann\thanks{Department of Applied Mathematics, Fictional University, Boise, ID 
	(\email{ptfrank@fictional.edu}, \email{jesmith@fictional.edu}).}
}
\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> tex/observability.tex <==
\section{Observability}
